Early Science with the Large Millimeter Telescope: an energy-driven wind revealed by massive molecular and fast X-ray outflows in the Seyfert Galaxy IRAS 17020+4544

We report on the coexistence of powerful gas outflows observed in millimeter and X-ray data of the Radio-Loud Narrow Line Seyfert 1 Galaxy IRAS 17020+4544. Thanks to the large collecting power of the Large Millimeter Telescope, a prominent line arising from the 12CO(1-0) transition was revealed in recent observations of this source. The complex profile is composed by a narrow double-peak line and a broad wing. While the double-peak structure may be arising in a disk of molecular material, the broad wing is interpreted as the signature of a massive outflow of molecular gas with an approximate bulk velocity of -660 km/s. This molecular wind is likely associated to a multi-component X-ray Ultra-Fast Outflow with velocities reaching up to ~0.1c and column densities in the range 10^{21-23.9} cm^-2 that was reported in the source prior to the LMT observations. The momentum load estimated in the two gas phases indicates that within the observational uncertainties the outflow is consistent with being propagating through the galaxy and sweeping up the gas while conserving its energy. This scenario, which has been often postulated as a viable mechanism of how AGN feedback takes place, has so far been observed only in ULIRGs sources. IRAS 17020+4544 with bolometric and infrared luminosity respectively of 5X10^{44} erg/s and 1.05X10^{11} L_sun appears to be an example of AGN feedback in a NLSy1 Galaxy (a low power AGN). New proprietary multi-wavelength data recently obtained on this source will allow us to corroborate the proposed hypothesis.

==> defs.tex <==
% Journal Definitions
\def\aa{AA}
\def\aap{AA}
\def\aj{AJ}
\def\apj{ApJ}
\def\apjl{ApJ}
\def\apjs{ApJS}
\def\mnras{MNRAS}
\def\araa{ARA\&A}
\def\nat{Nature}
%
% Common units
%
\def\arcsec{\ifmmode {''} \else ${''}$\fi}
\def\arcmin{\ifmmode {'} \else ${'}$\fi}
\def\deg{\ifmmode {^\circ} \else ${^\circ}$\fi}
\def\cc{\ifmmode {\rm cm}^{-3} \else cm$^{-3}$\fi}
\def\cl{\ifmmode {\rm cm}^{-2} \else cm$^{-2}$\fi}
\def\pcm2{\ifmmode {\rm cm}^{-2} \else cm$^{-2}$\fi}
\def\micron{\ifmmode \mu{\rm m} \else $\mu$m\fi}
\def\kms{\ifmmode {\rm km\,s}^{-1} \else km\,s$^{-1}$\fi}
\def\kmps{\ifmmode {\rm km\,s}^{-1} \else km\,s$^{-1}$\fi}
\def\Hubble{\ifmmode {\rm km\,s}^{-1}\,{\rm Mpc}^{-1}
        \else km\,s$^{-1}$\,Mpc$^{-1}$\fi}
\def\ergsec{\ifmmode {\rm ergs\;s}^{-1} \else ergs s$^{-1}$\fi}
\def\ergcms{\ifmmode {\rm ergs\,cm}^{-2}\,{\rm s}^{-1}
          \else ergs\,cm$^{-2}$\,s$^{-1}$\fi}
\def\ergcmsA{\ifmmode {\rm ergs\,cm}^{-2}\,{\rm s}^{-1}\,{\rm \AA}^{-1}
          \else ergs\,cm$^{-2}$\,s$^{-1}$\,\AA$^{-1}$\fi}
\def\ergcmsHz{\ifmmode {\rm ergs\,cm}^{-2}\,{\rm s}^{-2}\,{\rm Hz}^{-1}
          \else ergs\,cm$^{-2}$\,s$^{-1}$\,Hz$^{-1}$\fi}
%
% Solar units
%
\def\Msun{\ifmmode M_{\odot} \else $M_{\odot}$\fi}
\def\Lsun{\ifmmode L_{\odot} \else $L_{\odot}$\fi}
%
% Cosmological parameters
%
\def\qo{\ifmmode q_{0} \else $q_{0}$\fi}
\def\Ho{\ifmmode H_{0} \else $H_{0}$\fi}
%
% Approximately less than and greater than signs
%
\def\ltsim{\raisebox{-.5ex}{$\;\stackrel{<}{\sim}\;$}}
\def\gtsim{\raisebox{-.5ex}{$\;\stackrel{>}{\sim}\;$}}
%
% Line designations
%
\def\ion#1#2{#1$\;${\small\rm\@Roman{#2}}\relax}
\def\hi{H {\sc i}}
\def\Halpha{H$\alpha$}
\def\Hbeta{H$\beta$}
\def\Hgamma{H$\gamma$}
\def\Hdelta{H$\delta$}
\def\lya{Ly$\alpha$}
\def\lyb{Ly$\beta$}
\def\lyg{Ly$\gamma$}
\def\hei{He\,{\sc i}}
\def\cii{C\,{\sc ii}}
\def\ciii{C\,{\sc iii}}
\def\civ{C\,{\sc iv}}
\newcommand {\lm}{$\lambda$}
\newcommand {\etal}{et al.}
\newcommand {\hut}{{HUT}}
\newcommand{\oi}{O~{\sc i}}
\newcommand{\ovi}{O~{\sc vi}}
\newcommand{\ovii}{O~{\sc vii}}
\newcommand{\oviii}{O~{\sc viii}}
\newcommand{\heii}{He~{\sc ii}}
\newcommand{\feii}{Fe~{\sc ii}}
\def\oiii{{[O\,{\sc iii}]}}
\def\nv{N~{\sc v}}
\def\niii{N~{\sc iii}}
\def\siiv{Si~{\sc iv}}
\def\siiii{Si~{\sc iii}}
\def\siii{Si~{\sc ii}}
\def\fei{Fe\,{\sc i}}
\def\feii{Fe\,{\sc ii}}
\def\feiii{Fe\,{\sc iii}}
\def\feiv{Fe\,{\sc iv}}
\def\fexx{Fe\,{\sc xx}}
\def\hi{H\,{\sc i}}
\def\hii{H\,{\sc ii}}
\def\hei{He\,{\sc i}}
\def\heii{He\,{\sc ii}}
\def\ci{C\,{\sc i}}
\def\cii{C\,{\sc ii}}
\def\ciii{\ifmmode {\rm C}\,{\sc iii} \else C\,{\sc iii}\fi}
\def\civ{\ifmmode {\rm C}\,{\sc iv} \else C\,{\sc iv}\fi}
\def\cv{\ifmmode {\rm C}\,{\sc v} \else C\,{\sc v}\fi}
\def\cvi{\ifmmode {\rm C}\,{\sc vi} \else C\,{\sc vi}\fi}
\def\ni{N\,{\sc i}}
\def\nii{N\,{\sc ii}}
\def\niii{N\,{\sc iii}}
\def\niv{N\,{\sc iv}}
\def\nv{N\,{\sc v}}
\def\nvi{N\,{\sc vi}}
\def\nvii{N\,{\sc vii}}
\def\oi{O\,{\sc i}}
\def\oii{O\,{\sc ii}}
\def\oiii{O\,{\sc iii}}
\def\o5007{[O\,{\sc iii}]\,$\lambda5007$}
\def\oiv{O\,{\sc iv}}
\def\ov{O\,{\sc v}}
\def\ovi{O\,{\sc vi}}
\def\ovii{O\,{\sc vii}}
\def\oviii{O\,{\sc viii}}
\def\neiii{Ne\,{\sc iii}}
\def\nev{Ne\,{\sc v}}
\def\neviii{Ne\,{\sc viii}}
\def\neix{Ne\,{\sc ix}}
\def\nex{Ne\,{\sc x}}
\def\mgi{Mg\,{\sc i}}
\def\mnii{Mn\,{\sc ii}}
\def\Niii{Ni\,{\sc ii}}
\def\mgii{Mg\,{\sc ii}}
\def\mgix{Mg\,{\sc ix}}
\def\mgx{Mg\,{\sc x}}
\def\mgxi{Mg\,{\sc xi}}
\def\siiv{Si\,{\sc iv}}
\def\siIII{Si\,{\sc iii}}
\def\siII{Si\,{\sc ii}}
\def\six{Si\,{\sc x}}
\def\sixi{Si\,{\sc xi}}
\def\sixii{Si\,{\sc xii}}
\def\sixiii{Si\,{\sc xiii}}
\def\si{S\,{\sc i}}
\def\sii{S\,{\sc ii}}
\def\siii{S\,{\sc iii}}
\def\siv{S\,{\sc iv}}
\def\sv{S\,{\sc v}}
\def\svi{S\,{\sc vi}}
\def\sx{S\,{\sc x}}
\def\sxi{S\,{\sc xi}}
\def\sxii{S\,{\sc xii}}
\def\sxiii{S\,{\sc xiii}}
\def\ariii{Ar\,{\sc iii}}
\def\ariv{Ar\,{\sc iv}}
\def\arv{Ar\,{\sc v}}
\def\arvi{Ar\,{\sc vi}}
\def\arvii{Ar\,{\sc vii}}
\def\arviii{Ar\,{\sc viii}}
\def\caii{Ca\,{\sc ii}}
\def\fei{Fe\,{\sc i}}
\def\feii{Fe\,{\sc ii}}
\def\feiii{Fe\,{\sc iii}}
\def\feix{Fe\,{\sc ix}}
\def\fexvii{Fe\,{\sc xvii}}
\def\fexviii{Fe\,{\sc xviii}}
\def\fexix{Fe\,{\sc xix}}
\def\fexxiii{Fe\,{\sc xxiii}}
\def\fexxiv{Fe\,{\sc xxiv}}
\def\fexxv{Fe\,{\sc xxv}}
\def\fexxvi{Fe\,{\sc xxvi}}
\def\alii{Al\,{\sc ii}}
\def\aliii{Al\,{\sc iii}}
\def\piv{P\,{\sc iv}}
\def\cliv{Cl\,{\sc iv}}
\def\clv{Cl\,{\sc v}}
\def\nai{Na\,{\sc i}}
%
\def\fek{{\rm Fe\,K$\alpha$}}
\def\fekb{{\rm Fe\,K$\beta$}}
\def\xmm{XMM-{\it Newton}}
\def\chandra{{\it Chandra}}

